Cross-Domain Multi-Task Learning for Sequential Sentence Classification in Research Papers

Sequential sentence classification deals with the categorisation of sentences based on their content and context. Applied to scientific texts, it enables the automatic structuring of research papers and the improvement of academic search engines. However, previous work has not investigated the potential of transfer learning for sentence classification across different scientific domains and the issue of different text structure of full papers and abstracts. In this paper, we derive seven related research questions and present several contributions to address them: First, we suggest a novel uniform deep learning architecture and multi-task learning for cross-domain sequential sentence classification in scientific texts. Second, we tailor two common transfer learning methods, sequential transfer learning and multi-task learning, to deal with the challenges of the given task. Semantic relatedness of tasks is a prerequisite for successful transfer learning of neural models. Consequently, our third contribution is an approach to semi-automatically identify semantically related classes from different annotation schemes and we present an analysis of four annotation schemes. Comprehensive experimental results indicate that models, which are trained on datasets from different scientific domains, benefit from one another when using the proposed multi-task learning architecture. We also report comparisons with several state-of-the-art approaches. Our approach outperforms the state of the art on full paper datasets significantly while being on par for datasets consisting of abstracts.

==> img/highlight_example.tex <==
\begin{figure}[t]
\small
\centering%
\begin{tabular}{| p{\dimexpr0.47\textwidth-2\tabcolsep-\arrayrulewidth\relax}|   }
\hline
\\
Achilles tendinopathy (AT) is a common and difficult to treat musculoskeletal disorder.  The purpose of this study is to examine whether 1 injection of platelet-rich plasma (PRP) would improve outcomes more effectively than placebo (saline) after 3 months when used to treat AT. 
\colorbox{Yellow}{A total of 24 male patients with chronic AT (median disease duration, 33 months) were randomized (1:1) to receive either a blinded injection of PRP (n = 12) or saline (n = 12). Patients were informed that they could drop out after 3 months if they were dissatisfied with the treatment.} 
After 3 months, all patients were reassessed (no dropouts). No difference between the PRP and the saline group could be observed with regard to the primary outcome (VISA-A score: mean difference [MD], -1.3; 95\% CI, -17.8 to 15.2; P = .868). Secondary outcomes were pain at rest (MD, 1.6; 95\% CI, -0.5 to 3.7; P = .137), pain while walking (MD, 0.8; 95\% CI, -1.8 to 3.3; P = .544), pain when tendon was squeezed (MD, 0.3; 95\% CI, -0.2 to 0.9; P = .208).
PRP injection did not result in an improved VISA-A score over a 3-month period compared with placebo. 
The conclusions are limited to the 3 months after treatment owing to the large dropout rate. 
\\
\\
\hline
\end{tabular}
\caption{Example of abstract with the method section highlighted. Abstracts in the medical field can be long. This abstract was taken from~\protect\cite{krogh2016ultrasound} and several sentences have been removed for the sake of conciseness. Providing clinical researchers and practitioners a tool that would allow them to highlight the section(s) that
they are interested in would help them explore the literature more efficiently.}
\label{tab:highlight-example}
\end{figure}

